Patterns Count-Based Labels for Datasets

Counts of attribute-value combinations are central to the profiling of a dataset, particularly in determining fitness for use and in eliminating bias and unfairness. While counts of individual attribute values may be stored in some dataset profiles, there are too many combinations of attributes for it to be practical to store counts for each combination. In this paper, we develop the notion of storing a "label" of limited size that can be used to obtain good estimates for these counts. A label, in this paper, contains information regarding the count of selected patterns--attributes values combinations--in the data. We define an estimation function, that uses this label to estimate the count of every pattern. We present the problem of finding the optimal label given a bound on its size and propose a heuristic algorithm for generating optimal labels. We experimentally show the accuracy of count estimates derived from the resulting labels and the efficiency of our algorithm.

==> labels.tex <==
%!TEX root = ./main.tex

\section{Counting based labels}
\label{sec:labels}

We start by presenting a new model of nutrition label which is base on counts.
We assume the data is represented using a single relational database, and that the relation's attributes values are categorical. We start by defining the notion of pattern which plays a key rule in our labeling model. 


\begin{definition}[Patterns]
	Let $D$ be a database with attributes $\mathcal{A}=\{A_1,\ldots, A_n\}$ and let $Dom(A_i)$ be the active domain of $A_i$ for $i \in [1..n]$ . A \emph{pattern} $p$ over $D$  is set of $\{A_{i_1} = a_1, \ldots, A_{i_k} = a_k\}$ where $\{A_{i_1},,\ldots, A_{i_k}\}\subseteq \mathcal{A}$ and $a_j\in Dom(A_{i_j})$ for each $A_{i_j}$ in $p$. 
	
%	A \emph{full pattern} is a pattern $P$ that contains all $A_i\in \mathcal{A}$. We use $fp(D)$ to denote the set of all possible full patterns in the database $D$.
\end{definition}

\begin{example}
	Consider the  fragment of a simplified version of the COMPAS\cite{compas} database given in Figure \ref{fig:db}. It contains four categorical attributes: gender, age group, race and marital status. \{age group= under 20, marital status = singe\} is a possible pattern over  $S=$\{age group, marital status\}.  
\end{example}	
	
	\begin{definition}
	We say that a tuple $t\in D$ \emph{satisfies} a pattern $p$ if $t.A_i = a_i$ for each $A_i$ appearing in $p$.
	The count $c_D(p)$ of a pattern  $p$ is the number of tuples in $D$ that satisfy~$p$. 
%	We use $cp(D)$ to denote the set of all possible categories patterns over $D$. % with count greater than~$0$.
\end{definition}

\begin{example}
	Reconsider  the database given in Figure \ref{fig:db}. The tuples 1, 3, 8, 10, 12, and 14 satisfy the pattern $p=$\{age group= under 20, marital status = single\} and thus the count of~$p$~is~6.  
\end{example}	

\begin{figure}
	\centering
	\scriptsize
	\begin{tabular}{lcccc}
		%\cline{2-5}
		\hline
		&Gender & Age group & Race & Marital status\\ \hline % \cline{2-5}
		1&Female & under 20& African-American  & single\\
			2	&Male & 20-39& African-American & divorced\\
		3&Male & under 20& Hispanic  & single\\
		4&Male & 20-39& Caucasian & married\\
		5&Female & 20-39& African-American & divorced\\
			6	&Male & 20-39& Caucasian & divorced\\
		7&Female & 20-39& African-American & married\\
		8		&Male & under 20& African-American  & single\\
		9			&Female & 20-39& Caucasian & divorced\\
		10&Male & under 20& Caucasian  & single\\
		11&Male & 20-39& Hispanic & divorced\\
			12	&Female & under 20& Hispanic & single\\
		13&Female & 20-39& Hispanic & married\\
		14&Female & under 20& Caucasian & single\\
		15&Female & 20-39& Caucasian & married\\
			16	&Male & 20-39& Hispanic & married\\
		17&Male & 20-39& African-American & married\\
		18&Female & 20-39& Hispanic & divorced\\
		
		%			\cline{2-5}
		\hline
	\end{tabular}
	
	\caption{Sample data from a simplified version of the COMPAS dataset}
	\label{fig:db}
\end{figure}


Information regrading the count of patterns appearing in the data can be used to determine fitness of use, detect under represented groups, data skews and potentially correlation/dependence.

A simple yet important usage of patterns count is 

\paragraph*{Input Fairness Condition} 

\paragraph*{Underrepresented groups } 





\begin{itemize}
	\item Given the count of all patterns gives a detailed picture of the data
	\item give examples of usage: coverage and correlation
	\item problem: this information is too large and labels should be concise.
	 \item We next present bounded size labels and study the trade-off between label size and its accuracy.
\end{itemize}




While detailed and informative the patterns counts are, presenting users with such information may be overwhelming. A desirable and important feature of nutrition labels is their consciousness. This calls for a bounded size label solution, that naturally can not contains the full patterns count, but may be used to estimate the count of each pattern.

==> prelim.tex <==
    \section{Preliminaries}
\label{sec:prelim}

%Fairness


